Style Over Substance: Evaluation Biases for Large Language Models

As large language models (LLMs) continue to advance, accurately and comprehensively evaluating their performance becomes increasingly challenging. Ranking the relative performance of LLMs based on Elo ratings, according to human judgment, is gaining more popularity. However, the extent to which humans and LLMs are capable evaluators remains uncertain. This study investigates the behavior of crowd-sourced and expert annotators, as well as LLMs, when comparing outputs from different models. To achieve this, we curate a dataset of intentionally flawed machine-generated answers. Our findings reveal a concerning bias in the evaluation process, as answers with factual errors are rated more favorably than answers that are too short or contained grammatical errors. To address this issue, we propose independently evaluating machine-generated text across multiple dimensions, rather than merging all the evaluation aspects into a single score. We instantiate this idea with the Elo rating system, resulting in the Multi-Elo Rating System (MERS). Empirical results from our study reveal that this proposed approach significantly enhances the quality of LLM-based evaluations, particularly in terms of factual accuracy. However, there is no significant improvement in crowd-sourced-based evaluations, indicating the need for further investigation.

==> 4_llm.tex <==
\section{LLM-Based Evaluator Is Better Yet Not Good Enough}

\paragraph{LLM is a better evaluator}
% \input{tables/gpt4_all}
% \autoref{tab:gpt4_all}

\paragraph{GPT-4 prefers the first answer}


\paragraph{LLM still considers non-factual answers as good}

- non-factual is still better than short or ungrammatical.
- we check their reasoning, GPT4 notices the factual mistake, but still picks it as the best answer regardless.






==> 6_expert.tex <==
\section{Stop Using Crowd-Sourced Annotators!}

\input{tables/crowd_vs_expert}

In this section, we compare the behavior of crowd-sourced and expert annotators.

We organize a team of 20 expert annotators. Each the expert annotators at least has a master-level degree in an English-speaking country. We randomly sample 200 games and ask each of these experts to carefully annotate 10 games.\footnote{\url{https://new.uschess.org/frequently-asked-questions-member-services-area}}

==> figures/length_and_dist.tex <==
\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \scriptsize
    \begin{tikzpicture}
    \begin{axis}[
      xbar stacked,
      height=4cm,
      width=\textwidth,
      % enlargelimits=0.1,
      enlarge x limits={abs=0.2cm},
      enlarge y limits={abs=0.4cm},
      bar width=10pt,
      xmin=0, xmax=100,
      legend style={at={(0.5,-0.4)}, anchor=north,legend columns=1},
      legend cell align={left},
      xlabel={Percentage},
      symbolic y coords={Claude-1,GPT-4,Expert,Crowd},
      ytick=data,
      nodes near coords,
      every node near coord/.append style={font=\scriptsize},
      tick label style={font=\small},
      % nodes near coords align={horizontal},
      ]
    \addplot [xbar, fill=green!50, draw=green!50] coordinates {
    (66.8,Claude-1)
    (67.9,GPT-4)
    (51.9,Expert)
    (57.1,Crowd)
    };
    \addplot [xbar, fill=blue!50, draw=blue!50] coordinates {
    (33.2,Claude-1)
    (32.1,GPT-4)
    (48.1,Expert)
    (42.9,Crowd)
    };
    \legend{\texttt{Longer answer wins}, \texttt{Shorter answer wins}}
    \end{axis}
    \end{tikzpicture}
    \caption{
        The percentage distribution of decision choices made by humans and LLMs in terms of answer length (in words).
    }
    \label{fig:win_length}
\end{minipage}%
\hspace{5mm}
\begin{minipage}{.45\textwidth}
    \centering
    \scriptsize
    \begin{tikzpicture}
    \begin{axis}[
      xbar stacked,
      height=4cm,
      width=\textwidth,
      % enlargelimits=0.1,
      enlarge x limits={abs=0.2cm},
      enlarge y limits={abs=0.4cm},
      bar width=10pt,
      xmin=0, xmax=100,
      legend style={at={(0.5,-0.4)}, anchor=north,legend columns=1},
      legend cell align={left},
      xlabel={Percentage (\%)},
      symbolic y coords={Claude-1,GPT-4,Expert,Crowd},
      ytick=data,
      nodes near coords,
      every node near coord/.append style={font=\scriptsize},
      tick label style={font=\small},
      % nodes near coords align={horizontal},
      ]
    \addplot [xbar, fill=green!50, draw=green!50] coordinates {
    (52.6,Claude-1)
    (50.4,GPT-4)
    (35.5,Expert)
    (45.9,Crowd)
    };
    \addplot [xbar, fill=blue!50, draw=blue!50] coordinates {
    (44.6,Claude-1)
    (44.4,GPT-4)
    (44.5,Expert)
    (44.8,Crowd)
    };
    \addplot [xbar, fill=red!50, draw=red!50] coordinates {
    (2.8,Claude-1)
    (5.2,GPT-4)
    (20.0,Expert)
    (9.3,Crowd)
    };
    \legend{\texttt{Assistant 1 wins}, \texttt{Assistant 2 wins}, \texttt{Tie}}
    \end{axis}
    \end{tikzpicture}
    \caption{
        The distribution of decision choices made by humans and LLMs.
    }
    \label{fig:win_dist}
\end{minipage}
\end{figure}

==> figures/model_pair.tex <==



\begin{figure}[t]
    \centering
    \scriptsize
    \begin{tikzpicture}
    \begin{axis}[
      xbar stacked,
      height=4cm,
      width=0.4\textwidth,
      % enlargelimits=0.1,
      enlarge x limits={abs=0.2cm},
      enlarge y limits={abs=0.4cm},
      bar width=10pt,
      xmin=0, xmax=100,
      legend style={at={(0.5,-0.4)}, anchor=north,legend columns=1},
      legend cell align={left},
      xlabel={Percentage (\%)},
      symbolic y coords={Claude-1,GPT-4,Expert,Crowd},
      ytick=data,
      nodes near coords,
      every node near coord/.append style={font=\scriptsize},
      tick label style={font=\small},
      % nodes near coords align={horizontal},
      ]
    \addplot [xbar, fill=green!50, draw=green!50] coordinates {
    (93.8,Claude-1)
    (100,GPT-4)
    (100,Expert)
    (66.3,Crowd)
    };
    \addplot [xbar, fill=blue!50, draw=blue!50] coordinates {
    (5,Claude-1)
    (0,GPT-4)
    (0,Expert)
    (28.8,Crowd)
    };
    \addplot [xbar, fill=red!50, draw=red!50] coordinates {
    (1.2,Claude-1)
    (0,GPT-4)
    (0,Expert)
    (5.0,Crowd)
    };
    \legend{\texttt{``\correct'' wins}, \texttt{``\fewmajorerrorsandshort'' wins}, \texttt{Tie}}
    \end{axis}
    \end{tikzpicture}
    \caption{
        The distribution of decision choices made by humans and LLMs on the games between ``\correct'' and ``\fewmajorerrorsandshort''.
    }
    \label{fig:model_pair}
\end{figure}

==> tables/crowd_vs_expert.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcp{8mm}cp{8mm}cp{8mm}cp{8mm}cp{8mm}cp{8mm}}
\toprule
                & \multicolumn{4}{c}{Accuracy}                                                      & \multicolumn{4}{c}{Helpfulness}                                                         & \multicolumn{4}{c}{Language}                                                          \\ \cmidrule(rl){2-5} \cmidrule(rl){6-9} \cmidrule(l){10-13}
                & \multicolumn{2}{c}{Crowd}               & \multicolumn{2}{c}{Expert}              & \multicolumn{2}{c}{Crowd}                  & \multicolumn{2}{c}{Expert}                 & \multicolumn{2}{c}{Crowd}                 & \multicolumn{2}{c}{Expert}                \\ \midrule
\correct        & 1056           & \humanchart{1056}{59}{cyan} & 1180           & \humanchart{1180}{80}{cyan} & 1045           & \humanchart{1045}{58}{magenta} & 1208           & \humanchart{1208}{85}{magenta} & 1036           & \humanchart{1036}{56}{yellow} & 1109           & \humanchart{1109}{68}{yellow} \\
\quad + \texttt{Short}   & \phantom{0}963 & \humanchart{963}{44}{cyan}  & 1040           & \humanchart{1040}{57}{cyan} & \phantom{0}983 & \humanchart{983}{47}{magenta}  & \phantom{0}979 & \humanchart{979}{47}{magenta}  & 1007           & \humanchart{1007}{51}{yellow} & 1068           & \humanchart{1068}{61}{yellow} \\ \midrule
\oneminorerror  & 1026           & \humanchart{1026}{54}{cyan} & 1090           & \humanchart{1090}{65}{cyan} & 1048           & \humanchart{1048}{58}{magenta} & 1153           & \humanchart{1153}{76}{magenta} & 1019           & \humanchart{1019}{53}{yellow} & 1114           & \humanchart{1114}{69}{yellow} \\
\quad + \texttt{Short}   & \phantom{0}978 & \humanchart{978}{46}{cyan}  & \phantom{0}898 & \humanchart{898}{33}{cyan}  & \phantom{0}993 & \humanchart{993}{49}{magenta}  & \phantom{0}941 & \humanchart{941}{40}{magenta}  & \phantom{0}990 & \humanchart{990}{48}{yellow}  & 1012           & \humanchart{1012}{52}{yellow} \\
\fewminorerrors & 1036           & \humanchart{1036}{56}{cyan} & 1044           & \humanchart{1044}{57}{cyan} & 1051           & \humanchart{1051}{59}{magenta} & 1069           & \humanchart{1069}{62}{magenta} & 1029           & \humanchart{1029}{55}{yellow} & 1096           & \humanchart{1096}{66}{yellow} \\
\quad + \texttt{Short}   & \phantom{0}978 & \humanchart{978}{46}{cyan}  & \phantom{0}931 & \humanchart{931}{39}{cyan}  & \phantom{0}956 & \humanchart{956}{43}{magenta}  & \phantom{0}865 & \humanchart{865}{28}{magenta}  & \phantom{0}996 & \humanchart{996}{49}{yellow}  & \phantom{0}935 & \humanchart{935}{39}{yellow}  \\
\fewmajorerrors & 1030           & \humanchart{1030}{55}{cyan} & \phantom{0}963 & \humanchart{963}{44}{cyan}  & 1037           & \humanchart{1037}{56}{magenta} & 1015           & \humanchart{1015}{53}{magenta} & 1023           & \humanchart{1023}{54}{yellow} & 1010           & \humanchart{1010}{52}{yellow} \\
\quad + \texttt{Short}   & \phantom{0}955 & \humanchart{955}{43}{cyan}  & \phantom{0}787 & \humanchart{787}{15}{cyan}  & \phantom{0}940 & \humanchart{940}{40}{magenta}  & \phantom{0}766 & \humanchart{766}{11}{magenta}  & \phantom{0}982 & \humanchart{982}{47}{yellow}  & \phantom{0}879 & \humanchart{879}{30}{yellow}  \\ \midrule
\advanced       & 1028           & \humanchart{1028}{55}{cyan} & 1121           & \humanchart{1121}{70}{cyan} & 1032           & \humanchart{1032}{55}{magenta} & 1146           & \humanchart{1146}{74}{magenta} & 1004           & \humanchart{1004}{51}{yellow} & 1039           & \humanchart{1039}{57}{yellow} \\
\quad + \texttt{Short}   & \phantom{0}979 & \humanchart{979}{47}{cyan}  & \phantom{0}971 & \humanchart{971}{45}{cyan}  & \phantom{0}969 & \humanchart{969}{45}{magenta}  & \phantom{0}891 & \humanchart{891}{32}{magenta}  & \phantom{0}994 & \humanchart{994}{49}{yellow}  & \phantom{0}863 & \humanchart{863}{27}{yellow}  \\
\intermediate   & 1015           & \humanchart{1015}{53}{cyan} & 1076           & \humanchart{1076}{63}{cyan} & 1002           & \humanchart{1002}{50}{magenta} & 1095           & \humanchart{1095}{66}{magenta} & \phantom{0}991 & \humanchart{991}{49}{yellow}  & \phantom{0}992 & \humanchart{992}{49}{yellow}  \\
\quad + \texttt{Short}   & \phantom{0}956 & \humanchart{956}{43}{cyan}  & \phantom{0}898 & \humanchart{898}{33}{cyan}  & \phantom{0}945 & \humanchart{945}{41}{magenta}  & \phantom{0}872 & \humanchart{872}{29}{magenta}  & \phantom{0}930 & \humanchart{930}{38}{yellow}  & \phantom{0}884 & \humanchart{884}{31}{yellow}  \\ \bottomrule
\end{tabular}
\caption{
Elo ratings for different models with regard to ``Accuracy'', ``Helpfulness'', and ``Language'' given by crowd-sourced and expert annotators.
}
\label{tab:crowd_vs_expert}
\end{table*}

==> tables/model_pair_and_iaa.tex <==
\begin{table}[t]
\centering
  \begin{varwidth}{0.45\textwidth}
    \centering
    \scriptsize
    \begin{tabular}{lcccc}
    \toprule
             & \multicolumn{1}{l}{Crowd} & \multicolumn{1}{l}{Expert} & \multicolumn{1}{l}{GPT-4} & \multicolumn{1}{l}{Claude-1} \\ \midrule
    Crowd    & ---                       & 0.08                       & 0.11                      & 0.10                         \\
    Expert   & 0.08                      & ---                        & 0.09                      & 0.14                         \\
    GPT-4    & 0.11                      & 0.09                       & ---                       & 0.51                         \\
    Claude-1 & 0.10                      & 0.14                       & 0.51                      & ---                         \\ \bottomrule
    \end{tabular}
    \caption{Pairwise inter-annotator agreement measured by Cohen's kappa coefficient $\kappa$.}
    \label{tab:iaa}
  \end{varwidth}%
  \hspace{5mm}
  \begin{minipage}{0.45\textwidth}
    \centering
    \scriptsize
    \begin{tikzpicture}
    \begin{axis}[
      xbar stacked,
      height=4cm,
      width=\textwidth,
      % enlargelimits=0.1,
      enlarge x limits={abs=0.2cm},
      enlarge y limits={abs=0.4cm},
      bar width=10pt,
      xmin=0, xmax=100,
      legend style={at={(0.5,-0.4)}, anchor=north,legend columns=1},
      legend cell align={left},
      xlabel={Percentage (\%)},
      symbolic y coords={Claude-1,GPT-4,Expert,Crowd},
      ytick=data,
      nodes near coords,
      every node near coord/.append style={font=\scriptsize},
      tick label style={font=\small},
      % nodes near coords align={horizontal},
      ]
    \addplot [xbar, fill=green!50, draw=green!50] coordinates {
    (93.8,Claude-1)
    (100,GPT-4)
    (100,Expert)
    (66.3,Crowd)
    };
    \addplot [xbar, fill=blue!50, draw=blue!50] coordinates {
    (5,Claude-1)
    (0,GPT-4)
    (0,Expert)
    (28.8,Crowd)
    };
    \addplot [xbar, fill=red!50, draw=red!50] coordinates {
    (1.2,Claude-1)
    (0,GPT-4)
    (0,Expert)
    (5.0,Crowd)
    };
    \legend{\texttt{``\correct'' wins}, \texttt{``\fewmajorerrorsandshort'' wins}, \texttt{Tie}}
    \end{axis}
    \end{tikzpicture}
    \caption{
        The distribution of decision choices made by humans and LLMs on the games between ``\correct'' and ``\fewmajorerrorsandshort''.
    }
    \label{fig:model_pair}
  \end{minipage}
\end{table}
